On the Sample Complexity of Representation Learning in Multi-task Bandits with Global and Local structure

We investigate the sample complexity of learning the optimal arm for multi-task bandit problems. Arms consist of two components: one that is shared across tasks (that we call representation) and one that is task-specific (that we call predictor). The objective is to learn the optimal (representation, predictor)-pair for each task, under the assumption that the optimal representation is common to all tasks. Within this framework, efficient learning algorithms should transfer knowledge across tasks. We consider the best-arm identification problem for a fixed confidence, where, in each round, the learner actively selects both a task, and an arm, and observes the corresponding reward. We derive instance-specific sample complexity lower bounds satisfied by any $(\delta_G,\delta_H)$-PAC algorithm (such an algorithm identifies the best representation with probability at least $1-\delta_G$, and the best predictor for a task with probability at least $1-\delta_H$). We devise an algorithm OSRL-SC whose sample complexity approaches the lower bound, and scales at most as $H(G\log(1/\delta_G)+ X\log(1/\delta_H))$, with $X,G,H$ being, respectively, the number of tasks, representations and predictors. By comparison, this scaling is significantly better than the classical best-arm identification algorithm that scales as $HGX\log(1/\delta)$.

==> appB.1.LB_offline_insights.tex <==
% !TeX spellcheck = en_GB
% !TeX root=main_supplementary.tex
% !TeX encoding = UTF-8
\section{Sample Complexity: Lower Bound}

In this section, we first discuss the sample complexity lower bound, and then provide the proofs of Theorem \ref{thm:full_lower_bound_offline}, and of Propositions \ref{pro:1}-\ref{pro:2}. 

\subsection{Sample complexity lower bound: Intuition and differences with classical MAB}

{\bf Refactoring information.} To identify the optimal representation $g^\star$ as fast as possible, an algorithm should be able to perform \textit{information refactoring}, i.e., to use all the available information across tasks to estimate $g^\star$. To illustrate this concept, we use the model illustrated in Figure \ref{fig:symmetric_tasks}. In this model, there are only $2$ tasks $x_1,x_2$,  and $3$ arms in $\set{G}$ (and only $1$ arm in $\set{H}$, thus it can be ignored). For this model, to learn that $g_3$ is sub-optimal, we should mainly sample task $x_1$, since the gap between the rewards of $g^\star$ and $g_3$ is the largest. Similarly, learning that $g_2$ is sub-optimal should be mainly obtained by sampling task $x_2$. Using the same task, to infer that $g_2$ and $g_3$ are sub-optimal, would be much less efficient. This observation motivates the expression of our lower bound in Theorem \ref{thm:full_lower_bound_offline}.
\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\linewidth]{Figures/SampleComplexity/symmetric_tasks.png}
	\caption{Example of two symmetric tasks $x_1$ and $x_2$, where learning the optimal representation $g^\star$ can be accelerated by considering both tasks, instead of focusing only on a single task.}
	\label{fig:symmetric_tasks}
\end{figure}

{\bf Differences with the classical best-arm identification problem in MAB.} Another interesting fact, when compared to the classical MAB problem, is the computation of the most confusing problem $\lambda$ for the second inequality in Theorem \ref{thm:full_lower_bound_offline}. Consider the best-arm identification problem in MAB with $K$ arms. There the set of confusing problems is $\Lambda(\mu) = \{\lambda \in[0,1]^K: a^{\star}(\lambda)\neq a^{\star}(\mu)\}$, where $a^{\star}(\mu)$ denotes the optimal arm under $\mu$, i.e., $a^{\star}(\mu)=\argmax_{a\in K} \mu(a)$. The sample complexity lower bound derived for such classical MAB problems \cite{kaufmann2016complexity} exploits the fact that the set $\Lambda(\mu)$ can be written as follows:
\[\Lambda(\mu) = \bigcup_{a \neq a^{\star}(\mu)} \left\{\lambda \in [0,1]^K: \lambda_{a}>\lambda_{a^{\star}(\mu)} \right\}. \]
At this point, notice that the set $
\Lambda_a(\mu)=\left\{\lambda \in [0,1]^K: \lambda_{a}>\lambda_{a^{\star}(\mu)} \right\},a \neq a^\star(\mu),$ does not necessarily contain only models whose optimal arm is $a$. 
\begin{figure}[!h]
	\centering
	\includegraphics[width=1\linewidth]{Figures/SampleComplexity/sc-image.png}
	\caption{Example of set $\set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$. All points in the shadowed area are in the set. All arms above $m(x,\bar g, \bar h_x;\eta,\mu)$ must be changed and belong to $\set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$. In addition, $(\bar{g},\bar{h}_x)\in \set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$.}
	\label{fig:computation_confusing_problem}
\end{figure}
Unfortunately, this way of rewriting the set of confusing problems cannot be used in our problem setting. The reason is that we need to account for the model structure, i.e., the optimal representation $g^{\star}$ needs to be the same across all the tasks. Ignoring this constraint would result in an upper bound of the lower bound that we derived.

As a matter of fact, in classical MAB, to learn that $a$ is sub-optimal, the confusing parameters $\lambda\in \Lambda_a(\mu)$ differ from $\mu$ only for arms $a$ and $a^\star(\mu)$. Now in our case, confusing parameters need to differ from $\mu$ for more than 2 arms, as stated in Lemma \ref{lemma:second_ineq_solution_inner_opt}. When $\eta$ is fixed, to identify that $(\bar{g},\bar{h}_x)$ is sub-optimal, we need to change arms in the set $\set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$. Recall that: 
\[
\set{U}_{x,\bar g, \bar h_x}^\mu(\eta) \coloneqq \left\{(g',h') \in \mathcal{G}\times \mathcal{H}:  \mu(x,g',h') \geq \frac{\sum_{(g,h) \in \mathcal{N}_{x,g',h'}^\mu} \eta(x,g,h)\mu(x,g,h)} {\sum_{(g,h) \in \mathcal{N}_{x,g',h'}^\mu} \eta(x,g,h)} \right\}\cup \{\bar g, \bar h_x\},\]
	with $\mathcal{N}_{x,g,h}^\mu\coloneqq \{(g',h') \in \mathcal{G}\times \mathcal{H}: \mu(x,g',h')\geq \mu(x,g,h) \} \cup \{(\bar g, \bar h_x)\}$, and 
	\[ 
	m(x,\bar g, \bar h_x;\eta,\mu) =  \frac{\sum_{(g,h)\in \set U_{x,\bar g, \bar h_x}^\mu} \eta(x,g,h)\mu(x,g,h)}{\sum_{(g,h)\in \set U_{x,\bar g, \bar h_x}^\mu} \eta(x,g,h)},
	\]
The set $\set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$ can be computed easily by recursively enlarging the set. We start with a set with only $(g^\star,h_x^\star)$ and 
$(\bar{g},\bar{h}_x)$. We compute the corresponding value of $m(x,\bar g, \bar h_x;\eta,\mu)$, and if the latter does not comply with the definitions of the above sets, we add to the set $\set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$, the arm $(g,h)$ with the highest mean not already in the set. And we iterate until we have consistent definitions.

Figure \ref{fig:computation_confusing_problem} provides an illustration of the set $\set{U}_{x,\bar g, \bar h_x}^\mu(\eta)$, after the above procedure has stopped.
